Learning k-qubit Quantum Operators via Pauli Decomposition

Motivated by the limited qubit capacity of current quantum systems, we study the quantum sample complexity of $k$-qubit quantum operators, i.e., operations applicable on only $k$ out of $d$ qubits. The problem is studied according to the quantum probably approximately correct (QPAC) model abiding by quantum mechanical laws such as no-cloning, state collapse, and measurement incompatibility. With the delicacy of quantum samples and the richness of quantum operations, one expects a significantly larger quantum sample complexity. This paper proves the contrary. We show that the quantum sample complexity of $k$-qubit quantum operations is comparable to the classical sample complexity of their counterparts (juntas), at least when $\frac{k}{d}\ll 1$. This is surprising, especially since sample duplication is prohibited, and measurement incompatibility would lead to an exponentially larger sample complexity with standard methods. Our approach is based on the Pauli decomposition of quantum operators and a technique that we name Quantum Shadow Sampling (QSS) to reduce the sample complexity exponentially. The results are proved by developing (i) a connection between the learning loss and the Pauli decomposition; (ii) a scalable QSS circuit for estimating the Pauli coefficients; and (iii) a quantum algorithm for learning $k$-qubit operators with sample complexity $O(\frac{k4^k}{\epsilon^2}\log d)$.

==> GeneralClass.tex <==
 \section{More general Measurement Classes}
 \begin{definition}[Concentrated measurement classes] \label{def:eps concentrated around A}
Given $\epsilon\in [0,1]$ and a degree set $\mathcal{A}\subseteq \{0,1,2,3\}^d$, a concept class $\mathcal{C}$ is said to be $\epsilon$-concentrated around $\mathcal{A}$, if for each measurement $\mathcal{M}\in \mathcal{C}$ with $\gm=M_1-M_0$ as its operator representation, the following inequality holds $\sum_{\bfs\notin \mathcal{A}} \qgs^2\leq \epsilon^2,$ 
where $\qgs$ are the Fourier coefficients of $\gm$. 
\end{definition}

The classical counterpart of such classes has been studied extensively in the literature. Special cases of such classes are conjunctions, s-term DNF formulas \citep{Valiant1984},  half-spaces \citep{Kalai2005}, \textit{juntas} \citep{Mossel_ODonnell} and polynomial threshold functions \citep{Jackson1997}.
 
 \begin{definition} \label{def: compatible degree set}
Any subset $\mathcal{B}\subseteq \set{0,1,2,3}^d$ is said to be \textit{compatible} if all $\qps, \bfs\in\mathcal{B}$ mutually commute, i.e., $\qps \sigma^\bft - \sigma^\bft \qps=0, \forall \bft,\bfs \in \mathcal{B}$. Furthermore, a compatibility covering of a degree set $\mathcal{A}\subseteq \set{0,1,2,3}^d$ is a collection of distinct compatible subsets $\mathcal{B}_1, \mathcal{B}_2,\cdots, \mathcal{B}_m\subseteq \mathcal{A}$ for some $m\in \NN$ such that $\mathcal{A} = \medcup_{j=1}^m \mathcal{B}_j$.
\end{definition}
%This approach is related to  \textit{mutually unbiased observables} studied extensively to learn an operator \citep{Bandyopadhyay2001,Crawford2019,Lawrence2002}. 
Note that there always exists a covering, as the single-element subsets of $\mathcal{A}$ form a trivial one.  With the above definition, we present our second main result. 

 \begin{theorem}\label{thm: QLD general}
Let $\mathcal{C}$ be a concept class that is $\epsilon$-concentrated around a degree set $\mathcal{A}$, where $\epsilon \in [0,1]$. Then, there exists a quantum learning algorithm that  learns $\mathcal{C}$ with error up to
 \begin{align}\label{eq:sample complexity bound}
 2\opt_{\mathcal{C}}+2\epsilon + \order\bigg{\min_{\mathcal{B}_j~\text{covering of}~ \mathcal{A}}\sum_{j=1}^m \sqrt{ \frac{|\mathcal{B}_j|}{n}\log \frac{|\mathcal{B}_j|}{\delta}}}.
\end{align} 
 \end{theorem}

==> Pauli_Estimate.tex <==
\subsection{Estimating The Pauli Coefficients}\label{sebsec:Pauli Estimation}
%Idea: Compatibility cover + Priskle approach.
Based on Theorem \ref{thm:mislabeling prob}, it remains to find bounds on the sample size for estimating the Pauli coefficients. The no-cloning and state collapse postulates make the estimation process more difficult than the classical. In this section, we discuss the estimation process and derive bounds on the square loss. 

We start with estimating a single Pauli coefficient $\qfs$. For that we consider the POVM  $\qms := \{\Msopt_1, \Msopt_{-1} \}$ with outcomes in $\pmm$ and operators 
\begin{align}\label{eq:Ms operators}
\Msopt_{1} \deq \qps_+,\qquad \Lambda^\bfs_{-1} \deq \qps_-,
\end{align}
where $\qps$ is the Pauli operator corresponding to $\bfs\in \set{0,1,2,3}^d$ as in \eqref{eq:Pauly for s}. Moreover, $\qps_+$ and $\qps_-$ are the positive and negative part of $\qps$ (such that $\qps=\qps_+ - \qps_-$), constructed through the spectral decomposition of $\qps$.  With these definitions, $\qfs$ is estimated by measuring a set of $m$ samples with  $\qms$. Suppose, we only use $m<n$ samples.   Let $Z_i\in \pmm$ be the output of $\qms$ on the $i$th sample $(\rho_i, y_i), i=1,2,3..., m$. Then the estimation is computed as  $$\qfests = \frac{-1}{m2^d}\sum_{i=1}^m Z_i (-1)^{y_i}.$$
Figure \ref{fig:Estimation} demonstrates the estimation process for single coefficient. 

 From Born's rule, $Z_i$ is a binary random variable with bias $\tr{\qps_+ \rho_i}$. Hence, $\qfests$ itself is random.  In the following lemma we bound the estimation error. 
\begin{lem}\label{lem:estimating one qfs}
Let $\qfests = \frac{-1}{m2^d}\sum_i Z_i (-1)^{y_i}$, where $Z_i$ is the output of $\qms$ on the $i$th sample. Then, $\EE[\qfsest]=\qfs$. Moreover,  for any $\delta \in [0,1]$, with probability $(1-\delta)$ the estimation error satisfies: $$|\qfsest - \qfs| \leq \sqrt{\frac{8}{m}\log(2/\delta)}.$$
 \end{lem}

Note that we cannot use all the samples for estimating one coefficient; because the samples will be inaccessible as they collapse by the measurements. For learning $k$-qubit measurements, all the Pauli coefficients $\qps$, with $|\supp(\bfs)|\leq k$, need to be estimated. A combinatorial argument shows that there are at most $(1+\frac{d^{k-1}}{(k-1)!})4^k$ such coefficients. With naive, strategy one would partition the total $n$ samples into several equal size groups one for each coefficient. Hence, with Lemma \ref{lem:estimating one qfs}, the estimation loss satisfies
\begin{align*}
|\qfsest - \qfs| =  \order{\sqrt{\frac{4^kd^{k-1}}{(k-1)! n}\log(2/\delta)}},
\end{align*}
for all $\bfs, |\supp(\bfs)|\leq k$.


\begin{figure}[hbtp]
\centering
\includegraphics[scale=0.8]{Estimation.eps}
\caption{The process for estimating the Pauli coefficient $\qps$ of the labeling }
\label{fig:Estimation}
\end{figure}



\subsubsection{Compatibility}
To minimize the number of samples required for each estimation, we would like to measure as many observables as possible with shared samples. This is possible when $M_{\bfs}$ are mutually compatible. Note that each Pauli coefficient corresponds to an observable for measuring.  In that case, the idea is to first perform a fine-grained measurement $M_{\bfs}$ on the sample and then extract the estimations from additional post-measurement classical processes. Figure \ref{fig:compatible} demonstrates this idea, where $M_{ref}$ is the fine-grained measurement and $e$ represents the post-processing function. To check whether $M_\bfs$'s are compatible, we need the following result. 
  %However,  in general, this is not possible as the observables $M_{\bfs}$ might not be  \textit{compatible} with each other. 
%  That said, we elaborate on \textit{compatible} observables and present the following definition from \citep{Holevo2012}. 
%\input{QLD_Estimations.tex}


\begin{figure}[hbtp]
\centering
\includegraphics[scale=1]{CompatibleMeasuring.eps}
\caption{Measuring using compatible observables.}
\label{fig:compatible}
\end{figure}

\begin{definition} \label{def:compatible}
A set of observables $M_j=\{\Lambda^j_u: u\in \mathcal{U}\}, j=1,2,...,k$ are called \textit{compatible} if there exist a fine-grained measurement $M_{ref}=\set{A_w: w\in \mathcal{W}}$ and a function $e:\mathcal{W}\mapsto \mathcal{U}^k$ such that $\Lambda^j_u = \sum_{w\in \mathcal{W}: e(w)_j=u} A_w$ for all $u\in \mathcal{U}$ and all $j\in [k]$.
\end{definition}



%\begin{definition} \label{def:compatible}
%A set of observables $M_j=\{\Lambda^j_u: u\in \mathcal{U}\}, j=1,2,...,k$ are called \textit{compatible} if there exist a measurement $M_{ref}=\set{A_w: w\in \mathcal{W}}$ and a function $e:\mathcal{W}\mapsto \mathcal{U}^k$ such that $\Lambda^j_u = \sum_{w\in \mathcal{W}: e(w)_j=u} A_w$ for all $u\in \mathcal{U}$ and all $j\in [k]$.
%\end{definition}
%Not all $M_{\bfs}$'s are compatible.  For example, set $d=1$ and consider the Fourier observables $M_{\bfs_1}, M_{\bfs_2}$ and $M_{\bfs_3},$ where $\bfs_1=1, \bfs_2=2, \bfs_3=3$. %One can show that observable $M_{\bfs_1}$ is compatible with $M_{\bfs_3}$  but not with $M_{\bfs_2}$.
% \begin{remark}
%Note that not all $M_{\bfs}$'s are compatible.  For example, set $d=1$ and consider the Fourier observables $M_{\bfs_1}, M_{\bfs_2}$ and $M_{\bfs_3},$ where $\bfs_1=1, \bfs_2=2, \bfs_3=3$. One can show that observable $M_{\bfs_1}$ is compatible with $M_{\bfs_3}$  but not with $M_{\bfs_2}$. 
%\end{remark}
%To check whether $M_\bfs$'s are compatible, we need the following result. 
%Next, we characterize all sets of compatible $M_{\bfs}$'s. 
%Since our Fourier observables are sharp we can characterize all sets of compatible $M_{\bfs}$'s. 
%\begin{proposition}\label{prop:compatible Ms}
%Given a set $\mathcal{A}\subseteq \set{0,1,2,3}^d$, the  observables  $M_{\bfs}, \bfs\in\mathcal{A}$ are compatible if and only if  the operators $\qps, \bfs\in \mathcal{A}$  mutually commute, or equivalently $\sigma^{\bfs}\sigma^{\bft}=\sigma^{\bft}\sigma^{\bfs}$ for all $\bfs, \bft\in \mathcal{A}$. 
%\end{proposition}
%\begin{proof}
% Since $M_{\bfs}$'s are sharp, then from  Theorem 2.13 of \citep{Holevo2012} they are compatible if and only if their operators commute, that is  $\Lambda_{z}^{\bfs}$ in \eqref{eq:Ms operators} must commute for all $\bfs \in\mathcal{A}$ and $z\in \pmm$. Since, $\Msopt_{-1}=I-\Msopt_1$, then the commutativity  condition is equivalent to say that $\Msopt_1\Lambda^{\bft}_1=\Lambda^{\bft}_1\Msopt_1$ for for all $\bfs, \bft\in \mathcal{A}$. Note that $\qps$ and $\qfY$ in \eqref{eq:Ms operators} commute. Therefore, $\Msopt_1$ and $\Lambda^{\bft}_1$ commute if and only if $\qps$ and $\sigma^{\bft}$ commute. With that, the proof is complete.    
%\end{proof}
%The result is a consequence of Theorem 2.13 of \citep{Holevo2012}. 
%The detailed argument for the proof is given in Appendix \ref{app:prop:compatible Ms}. 

%Now we are ready to explain the estimation process for a  compatible degree set $\mathcal{A}$. 
Consider a set $\mathcal{A}$ so that  $M_{\bfs}, \bfs\in\mathcal{A}$ are all compatible. From Definition \ref{def:compatible}, we can obtain these observables via a fine-grained measurement $M_{ref}$ and a function $e$. In what follows, we construct such elements. 

Without loss of generality, let $\mathcal{A}= \set{\bfs_1, \bfs_2, \cdots, \bfs_m}$ for some $m\in \NN$. Then, we construct $M_{ref}=\{\Gamma_{\bfw}: \bfw\in \pmm^m\}$ with the operators
{  \begin{align}\label{eq:Mref opt}
\Gamma_{\bfw} = \prod_{\ell=1}^m \Lambda^{\bfs_\ell}_{w_\ell} , \qquad  \text{for all}~ \bfw\in \pmm^m, 
\end{align} }
where $\Lambda^{\bfs_\ell}_{w_\ell}$ are the operators given in \eqref{eq:Ms operators}. By construction,  $M_{ref}$ is a valid sharp POVM. With that, the function $e$ is simply the identity function on $\pmm^m$, that is $e(\bfw)=\bfw,$ for all $\bfw\in \pmm^m$.  Therefore, the estimation process is as follows: We perform $M_{ref}$ on each sample. Let $\bfW_i, i\in [n]$ be the outcome of this measurement on the $i$th sample. Then, to estimate $f_{\bfs_\ell}$, we compute the empirical mean 
{  \begin{align}\label{eq:qfsest compatible}
\hat{f}_{\bfs_\ell}  = \frac{1}{n}\sum_{i=1}^n W_{i,\ell},\qquad \text{for all} ~\ell\in [m],
\end{align} }
where $W_{i,\ell}$ is the $\ell$th component of $\bfW_i$. %Hence, we obtain our estimation process presented as Procedure   \ref{proc:FourierEstimation}. % can simultaneously estimate these Fourier coefficients without the need for fresh batches of samples.  
%We derive the following bound on the estimation error.
In this case, it is not difficult to show that, for $\delta\in [0,1]$,  the  inequality  
$$\sup_{\bfs \in \mathcal{A}} |\qfsest - \qfs| = \order{ \sqrt{\frac{1}{n}\log \frac{|\mathcal{A}|}{\delta}}},$$
holds with probability at least $(1-\delta)$.
%

Compared to the naive strategy with fresh copy for each coefficient, we get exponential improvements when $\mathcal{A}$ is compatible. %In this case, with Lemma \ref{lem:compatible A fourier est}, the square loss of the Fourier estimations is less than $\beta^2=\frac{8|\mathcal{A}|}{n}\log \frac{2|\mathcal{A}|}{\delta}$ as needed in Theorem \ref{thm: QLD Predictor only}. %Now, if $\mathcal{A}$ is not compatible, we need compatible covering that is explained in the next section.

For learning $k$-qubit measurements, our set of coefficients are not mutually compatible. Let $\mathcal{B}_k=:\set{\bfs: |\supp(\bfs)|\leq k}$. In this case, we partition $\mathcal{B}$ into compatible subsets denoted by $\mathcal{A}_1, \mathcal{A}_2, \cdots, \mathcal{A}_m$ so that $\mathcal{B}_k=\medcup_i \mathcal{A}_i$. Furthermore, we divide the samples into $m$ groups one for each compatible subset. With this approach, we obtain the following bound

$$
 \sup_{\bfs: |\supp(\bfs)|\leq k} |\qfsest - \qfs| = \order{\min_{\mathcal{A}_j: j\in [m]~}\sum_{j=1}^m \sqrt{ \frac{1}{n}\log \frac{|\mathcal{B}_j|}{\delta}}}.$$
 In what follows, we derive bounds on this quantity. For that it remains to characterize sets of compatible observables $M_{\bfs}$.
 
\subsubsection{Bounds on Compatibility}

 Consider a fixed coordinate $\mathcal{J}$ with size $k$. There are $4^k$ Pauli operators on that coordinate. We try to find the sets of compatible ones among that group. For that we need the notion of mutually unbiased bases. 
%Now the question is to find the compatible sets of observables.
\begin{definition}
Let $\mathcal{B}_1 = \set{\ket{\phi_1}, \ket{\phi_2}, ..., \ket{\phi_m}}$ and $\mathcal{B}_2 = \set{\ket{\psi_1}, \ket{\psi_2}, ..., \ket{\psi_m}}$ two orthonormal bases in a Hilbert space of dimension $m$. Then, $\mathcal{B}_1$ and $\mathcal{B}_2$ are said to be mutually unbiased bases (MUB) if $\braket{\phi_i}{\psi_j}=\frac{1}{\sqrt{m}}$ for all $i, j \in [m]$. 
\end{definition}

Given coordinate system $\mathcal{J}$, each Pauli operator $\qps$ with $\supp(\bfs)\subseteq \mathcal{J}$ corresponds to an orthonormal basis in the $\mathcal{J}$ Hilbert space.  As the dimension of this space is $2^k$, there are at most $2^k+1$ MUB basis based on the Pauli operators \citep{Bandyopadhyay2001}. Hence, out of the $4^k$ sets of Pauli operators, there are $2^k+1$ distinct sets of MUB bases, where inside each set there are $2^k-1$ mutually commuting Pauli operators   \citep{Lawrence2002}.  
%In the Hilbert space corresponding to the coordinate system $\mathcal{J}$, there are $2^k$ groups of mutually compatible Paulies. 3
Therefore,  all the Pauli coefficients can be estimated with error up to 
\begin{align*}
\order{\sqrt{\frac{k d^k}{n}\log \frac{1}{\delta}}}.
\end{align*}
 
%\begin{procedure}[h]
%\caption{FourierEstimation() in QLD algorithm}\label{proc:FourierEstimation}
%\DontPrintSemicolon
% \SetKwProg{Fn}{Function}{:}{} 
% \SetKwProg{Est}{Estimation}{ (\emph{Batch} $j$, $\mathcal{B}_j$):}{}
% \Fn{\FourierEstimation{$\mathcal{B}_j, j\in [m]$}}{
% %Take the optimal covering of $\mathcal{A}$ denoted by $\mathcal{B}_j, j\in [m]$.\;
% Partition the samples into $m$ bathes, each of size $n_j^*, j\in [m]$, as in Lemma \ref{lem:optimal nj for covering }.\;
% 
%    \For{$j=1$ \KwTo $m$}{
% %%\Est{}{  
%  \addvd{  On samples in the $j$th batch apply POVM $M^j_{ref}$ with operators  in \eqref{eq:Mref opt} and $\bfs_\ell\in \mathcal{B}_j$. \;}
%%Apply $M^j_{ref}$ on each sample in the $j$th batch. \;
%Compute the empirical Fourier coefficient $\qfsest$ for all $\bfs\in\mathcal{B}_j$,  as in \eqref{eq:qfsest compatible}. \;
%   }
%   \KwRet $\qfsest$ for all $\bfs\in\mathcal{A}$
%   }
   
%\Fn{\FourierEstimation{$\mathcal{A}$}}{
% Construct the POVM $M_{ref}$ with operators as  in \eqref{eq:Mref opt}. \;
%Apply $M_{ref}$ on each sample. \;
%Compute the empirical Fourier coefficient $\qfsest$ for all $\bfs\in\mathcal{A}$,  as in \eqref{eq:qfsest compatible}. \;
%\KwRet $\qfsest, \bfs \in \mathcal{A}$\;
%}
%\end{procedure} 

{\color{red} With Shadow Tomography and \citep{Huang2020}: the bound might reduced to 
\begin{align*}
\order{\sqrt{\frac{k \log d}{n}\log \frac{1}{\delta}}}.
\end{align*}}
%\addvd{Note that the running time of this procedure is $\order{n 4^{|\mathcal{A}|}}$, as there are $4^{|\mathcal{A}|}$ that many Fourier coefficients to estimate. Moreover, the running time of Algorithm \ref{alg: QLD general} is also dominated by this term.}   Lastly, we point out that in QLD algorithm, the set $\mathcal{A}$ is given as an input. Whether the optimal loss $\opt_{\mathcal{C}}$ of a concentrated class with degree set $\mathcal{A}$ is lower than another concentrated class with a different degree set is in general open. In the next section, we answer this question for a special type of concentrated measurement classes. 


%\subsection{Constructing the predictor}

  {  \begin{algorithm}[h]
\caption{Algorithm for  $k$-qubit Circuits}
\label{alg: QLD juntas}
\DontPrintSemicolon
%\LinesNumbered
\KwIn{$k$, covering $\mathcal{A}_j, j\in [m]$,  and $n$ quantum training samples.}
\KwOut{Predictor $\hat{\mathcal{M}}$}
 \SetKwProg{Fn}{}{:}{} 
% \SetKwFunction{Compatible}{Compatibility Covering}
 \SetKwFunction{Junta}{Process:}
 %\SetKwFunction{Predictor}{Predictor}
% \SetKwFunction{FEST}{FourierEstimation}
\Fn{\Junta}{
%Let  $\mathcal{A}_j, j\in [m]$ be the optimal covering of $\mathcal{B}_k.$\;
%Run  \FourierEstimation{$\mathcal{B}_j, j\in [m]$}.\;
Divide the training samples into $m$ groups.\;
For each $\mathcal{A}_j$, estimate the Pauli coefficients $\qfs, \bfs \in \mathcal{A}_j$ using \eqref{eq:qfsest compatible}.\;
For each $\mathcal{J}\subset [d]$ with $|\mathcal{J}|=k$,  compute $\norm\big{\qfYestJ}_{1,\rho}$, where $\qfYestJ= \sum_{\bfs: \supp(\bfs)\subseteq \mathcal{J}} \qfsest \qps$ and find $\hat{\mathcal{J}}$ that maximizes it.\; %and find $\hat{\mathcal{J}}$ that maximizes the 1-norm. \;
Construct the projector $\PiJ$ as in \eqref{eq:Pi k} with $\mathcal{J}=\hat{\mathcal{J}}$.\;
 \KwRet  POVM $\hat{\mathcal{M}}:=\{\PiJ, I-\PiJ\}$ as the predictor. 
}
\end{algorithm} }

Lastly with this bound and Theorem \ref{thm:loss M_k}, we establish our main result presented as in Theorem \ref{thm: Kjunta sample complexity}. Moreover, the procedure is summarized as Algorithm \ref{alg: QLD juntas}.
 
 {\color{red} New bound with shadow tomography might look like
\begin{align*}
\opt_{k}+\order{ \sqrt{ \frac{k\log d}{n}\log \frac{1}{\delta}}}.
\end{align*}}

==> QLD_Estimations.tex <==
%\subsubsection{Estimation Process}\label{subsec: estimation}
 %The estimation process is done by applying appropriately designed quantum measurements on the samples. As stated in the introduction, 
 %However, due to the quantum nature of the problem, such an approach is not straightforward and there are challenges to be resolved. First, after performing a measurement,  the quantum state of the sample collapses and cannot be used for further processes/estimations.   
%Second,
% the observables corresponding to the Fourier coefficients may not be \textit{compatible} and hence the \textit{uncertainty principle} limits the accuracy of estimations  \citep{Holevo2012}.  That said, we start with defining the quantum observables for each Fourier coefficient. We show how to approximate a single Fourier coefficient from the quantum samples. We then focus on the \textit{compatibility} issue. %Next, we consider estimating compatible Fourier coefficients. 
%We address the second issue subsection \ref{subsec:general set}.  For that, we design a refined measurement followed by a set of classical post-measurement processes. We start with estimating a single Fourier coefficient.  Then, we propose QLD  for such sets and analyze their learning performance.      
%, due to the no-cloning theorem, it is impossible to reuse the samples in general. 

 % some challenges need to be addressed. First,  This is in contrast to the classical setting.



%due to We will propose a similar idea in our quantum learning framework. The idea is to design and apply quantum measurements to estimate the quantum Fourier coefficients.  However, such an approach is not straightforward as the training samples are quantum states.  Hence, one needs to appropriately design a collection of POVM's to estimate the Fourier coefficients.   
%In what follows, we describe our method. The objective is to estimate a set of Fourier coefficients $\qfs$ defines as $\qfs=\tr{\qps\qfY\rho_{XY}}$.

%\subsubsection{Estimating one Fourier Coefficient}\label{subsec:estimating one fq}
% $M_\bfs = \{\Msopt_1, \Msopt_{-1} \}$, where 
%\begin{align}\label{eq:Ms operators}
%\Msopt_{1} \deq \frac{1}{2}(\id + \qps \qfY),\qquad \Lambda^\bfs_{-1} \deq \frac{1}{2}(\id - \qps \qfY),
%\end{align}
%where the measurement's outcome belongs to $\pmm$, and  $\qps$ is the Pauli operator corresponding to $\bfs$ as in \eqref{eq:Pauly for s}. It is not difficult to check that $M_{\bfs}$ is a valid sharp POVM. 
\begin{definition} 
For any $\bfs\in \set{0,1,2,3}^d$, the quantum observable for estimating the Fourier coefficient $\qfs$ is defined as the POVM $M_\bfs := \{\Msopt_1, \Msopt_{-1} \}$ with outcomes $\pmm$ and operators 
\begin{align}\label{eq:Ms operators}
\Msopt_{1} \deq \frac{1}{2}(\id + \qps \qfY),\qquad \Lambda^\bfs_{-1} \deq \frac{1}{2}(\id - \qps \qfY),
\end{align}
where $\qps$ is the Pauli operator corresponding to $\bfs$ as in \eqref{eq:Pauly for s}.  
\end{definition}
%Note that $\qps$ and $\qfY$ commute. Therefore, $\qps \qfY$ is a valid quantum Boolean function as the following equations hold:
%\begin{align*}
%(\qps\qfY)^\dagger &=  \qfY^\dagger (\qps)^\dagger = \qfY\qps = \qps \qfY\\
%(\qps\qfY)^2&=\qps\qfY \qps\qfY = \qps\qps\qfY\qfY = \id.
%\end{align*}
%As a result, $\Pi_\bfs$ is a projection operator and hence, $M_\bfs$ is a valid POVM. 
%Now let $Z$ be the classical output when $M_\bfs$ applies to $\rho_{XY}$.  Note that $Z$ is a Bernoulli random variable with
%\begin{align*}
%\EE[Z] = \prob{Z=1} = \tr{\Lambda_1\rho_{XY}} = \frac{1}{2}-\frac{1}{2} \tr{\qps\qfY\rho_{XY}}. 
%\end{align*}
%Therefore, $\qfs =1-2\EE[X]$. Hence, we need to estimate the expected value of $Z$. 
We measure each sample $\rho_{y_i}\tensor \ketbra{y_i}, i\in [n]$ using $M_\bfs$. Let $Z_i\in \pmm$ be the output of the measurement on the $i$th sample. Note that even when the samples are fixed, $Z_i$'s are still random variables. These random variables are connected to $\qfs$ via the following lemma. %which is proved in Appendix \ref{app:lem:estimating one qfs}.



\begin{lem}\label{lem:estimating one qfs}
For any $\bfs\in \set{0,1,2,3}^d$ and $i\in [n]$, the outcome of  $M_{\bfs}$ on the $i$th sample is a random variable $Z_i$ with $\EE[Z_i] = \qfs$, where $\qfs$ is the Fourier coefficient of $\qfY$ and the expectation is taken with respect to the overall randomness induced by the measurement and the  sample's distribution. % \footnote{More precisely, it is understood that $\EE[Z] = \EE_\mu[\<M_{\bfs}\>_{i},$ where $\mu$ is the distribution of the random sample on the algebra of linear operators and $\<M_{\bfs}\>_i$ is the expectation value of the observable in the $i$th sample.}.
\end{lem}
\input{proof_lem_estimating_qfs.tex}

Note that since the samples are \ac{iid}, then so are $Z_i$'s. Hence,  to estimate $\qfs$, we need to approximate the expected value of these random variables. This is done by computing the empirical mean $\qfsest = \frac{1}{n}\sum_i z_i$ and the empirical sum converges to the expectation which is $\qfs$. To show this we have the following result which is a quantum analogous of Chernoff-Hoeffding's inequality.

\begin{lem}\label{lem:quantum chernoff}
Let $\rho_1, \rho_2, ..., \rho_n$ be \ac{iid} random density operators on a finite dimensional Hilbert space $H$. Let $\bar{\rho}=\EE[\rho_i]$ be the corresponding average density operator.\footnote{Equivalently, $\rho_i$'s are \textit{operator-valued} random variables with values in $\mathcal{D}(H)$, the \textit{algebra} of linear operators on $H$, that are self-adjoint, non-negative, and unite-trace.}  Let $\mathcal{M}$ be a (discrete) observable on $H$ with outcomes  belonging to $[a,b]$, where $a,b\in \RR$. If $Z_i$ is the  outcome for measuring $\rho_i$, then for any $t\geq  0$
  \begin{align*}
\prob{\abs\Big{\frac{1}{n}\sum_{i=1}^n Z_i - \<\mathcal{M}\>_{\bar{\rho}}} \geq t }\leq 2 \exp{-\frac{nt^2}{2(b-a)^2}}, 
\end{align*} 
   where $\<M\>_{\bar{\rho}}$ is the \textit{expectation value} of $\mathcal{M}$ in the average state $\bar{\rho}$.  
\end{lem}
The proof is omitted as it is a direct consequence of Theorem A.19 in   \citep{Ahlswede2002}.
From Lemma \ref{lem:quantum chernoff}, with $a=-1, b=1$,  we obtain that 
$$ \prob{|\qfsest - \qfs| \geq t}\leq 2\exp{-\frac{1}{8}nt^2}.
$$
Hence, given $\delta \in [0,1]$, with probability $(1-\delta)$ the following inequality holds $$|\qfsest - \qfs| \leq \sqrt{\frac{8}{n}\log(2/\delta)}.$$

\noindent\textbf{Naive extension to multiple coefficients:} A naive method to estimate all Fourier coefficients $\qfs, \bfs\in \mathcal{A}$ is to repeat the above process on fresh batches of samples. For that, the samples are partitioned into $|\mathcal{A}|$ batches of equal size, one batch for each $\bfs\in \mathcal{A}$. %Then, we apply the observable $M_{\bfs}$ on all the samples inside the corresponding group and calculate the empirical mean as in the single Fourier estimation. 
For this strategy, with $n$ samples, it is not difficult to see that, the estimation error is bounded as $$\sup_{\bfs\in \mathcal{A}} |\qfsest - \qfs| \leq \sqrt{ \frac{8|\mathcal{A}|}{n}\log\frac{2}{\delta}}.$$
 
 
%\subsubsection{Compatibility Issue} 
\subsubsection{Estimating \textit{Compatible} Fourier Coefficients}\label{subsec:compatibility}

To minimize the number of samples required for each estimation, we would like to measure as many observables as possible on one sample. This is possible when $M_{\bfs}, \bfs\in \mathcal{A}$ are compatible. In that case, the idea is to first perform a fine-grained measurement $M_{\bfs}$ on the sample and then extract the estimations from additional post-measurement classical processes. Figure \ref{fig:compatible} demonstrates this idea, where $M_{ref}$ is the fine-grained measurement and $e$ represents the post-processing function. To check whether $M_\bfs$'s are compatible, we need the following result. 
  %However,  in general, this is not possible as the observables $M_{\bfs}$ might not be  \textit{compatible} with each other. 
%  That said, we elaborate on \textit{compatible} observables and present the following definition from \citep{Holevo2012}. 
\begin{figure}[hbtp]
\centering
\includegraphics[scale=1]{CompatibleMeasuring.eps}
\caption{Measuring using compatible observables.}
\label{fig:compatible}
\end{figure}



%\begin{definition} \label{def:compatible}
%A set of observables $M_j=\{\Lambda^j_u: u\in \mathcal{U}\}, j=1,2,...,k$ are called \textit{compatible} if there exist a measurement $M_{ref}=\set{A_w: w\in \mathcal{W}}$ and a function $e:\mathcal{W}\mapsto \mathcal{U}^k$ such that $\Lambda^j_u = \sum_{w\in \mathcal{W}: e(w)_j=u} A_w$ for all $u\in \mathcal{U}$ and all $j\in [k]$.
%\end{definition}
%Not all $M_{\bfs}$'s are compatible.  For example, set $d=1$ and consider the Fourier observables $M_{\bfs_1}, M_{\bfs_2}$ and $M_{\bfs_3},$ where $\bfs_1=1, \bfs_2=2, \bfs_3=3$. %One can show that observable $M_{\bfs_1}$ is compatible with $M_{\bfs_3}$  but not with $M_{\bfs_2}$.
% \begin{remark}
%Note that not all $M_{\bfs}$'s are compatible.  For example, set $d=1$ and consider the Fourier observables $M_{\bfs_1}, M_{\bfs_2}$ and $M_{\bfs_3},$ where $\bfs_1=1, \bfs_2=2, \bfs_3=3$. One can show that observable $M_{\bfs_1}$ is compatible with $M_{\bfs_3}$  but not with $M_{\bfs_2}$. 
%\end{remark}
%To check whether $M_\bfs$'s are compatible, we need the following result. 
%Next, we characterize all sets of compatible $M_{\bfs}$'s. 
%Since our Fourier observables are sharp we can characterize all sets of compatible $M_{\bfs}$'s. 
\begin{proposition}\label{prop:compatible Ms}
Given a set $\mathcal{A}\subseteq \set{0,1,2,3}^d$, the  observables  $M_{\bfs}, \bfs\in\mathcal{A}$ are compatible if and only if  the operators $\qps, \bfs\in \mathcal{A}$  mutually commute, or equivalently $\sigma^{\bfs}\sigma^{\bft}=\sigma^{\bft}\sigma^{\bfs}$ for all $\bfs, \bft\in \mathcal{A}$. 
\end{proposition}
\begin{proof}
 Since $M_{\bfs}$'s are sharp, then from  Theorem 2.13 of \citep{Holevo2012} they are compatible if and only if their operators commute, that is  $\Lambda_{z}^{\bfs}$ in \eqref{eq:Ms operators} must commute for all $\bfs \in\mathcal{A}$ and $z\in \pmm$. Since, $\Msopt_{-1}=I-\Msopt_1$, then the commutativity  condition is equivalent to say that $\Msopt_1\Lambda^{\bft}_1=\Lambda^{\bft}_1\Msopt_1$ for for all $\bfs, \bft\in \mathcal{A}$. Note that $\qps$ and $\qfY$ in \eqref{eq:Ms operators} commute. Therefore, $\Msopt_1$ and $\Lambda^{\bft}_1$ commute if and only if $\qps$ and $\sigma^{\bft}$ commute. With that, the proof is complete.    
\end{proof}
%The result is a consequence of Theorem 2.13 of \citep{Holevo2012}. 
%The detailed argument for the proof is given in Appendix \ref{app:prop:compatible Ms}. 

Now we are ready to explain the estimation process for a  compatible degree set $\mathcal{A}$. Suppose $M_{\bfs}, \bfs\in\mathcal{A}$ are all compatible. From Definition \ref{def:compatible}, we can obtain these observables via a fine-grained measurement $M_{ref}$ and a function $e$. In what follows, we construct such elements. 

Without loss of generality, let $\mathcal{A}= \set{\bfs_1, \bfs_2, \cdots, \bfs_m}$ for some $m\in \NN$. Then, we construct $M_{ref}=\{\Gamma_{\bfw}: \bfw\in \pmm^m\}$ with the operators
{  \begin{align}\label{eq:Mref opt}
\Gamma_{\bfw} = \prod_{\ell=1}^m \Lambda^{\bfs_\ell}_{w_\ell} , \qquad  \text{for all}~ \bfw\in \pmm^m, 
\end{align} }
where $\Lambda^{\bfs_\ell}_{w_\ell}$ are the operators given in \eqref{eq:Ms operators}. By construction,  $M_{ref}$ is a valid sharp POVM. With that, the function $e$ is simply the identity function on $\pmm^m$, that is $e(\bfw)=\bfw,$ for all $\bfw\in \pmm^m$.  Therefore, the estimation process is as follows: We perform $M_{ref}$ on each sample. Let $\bfW_i, i\in [n]$ be the outcome of this measurement on the $i$th sample. Then, to estimate $f_{\bfs_\ell}$, we compute the empirical mean 
{  \begin{align}\label{eq:qfsest compatible}
\hat{f}_{\bfs_\ell}  = \frac{1}{n}\sum_{i=1}^n W_{i,\ell},\qquad \text{for all} ~\ell\in [m],
\end{align} }
where $W_{i,\ell}$ is the $\ell$th component of $\bfW_i$. %Hence, we obtain our estimation process presented as Procedure   \ref{proc:FourierEstimation}. % can simultaneously estimate these Fourier coefficients without the need for fresh batches of samples.  
We derive the following bound on the estimation error. 
\begin{lem}\label{lem:compatible A fourier est}
Let $\mathcal{A}\subseteq\set{0,1,2,3}^d$ be a set such that $M_{\bfs}, \bfs\in \mathcal{A}$ are compatible. Let $\qfsest, \bfs\in \mathcal{A}$ be the empirical estimates of $\qfs$ as in  \eqref{eq:qfsest compatible} and using $n$ quantum samples. Then, for $\delta\in [0,1]$,  the  inequality  
$$\sup_{\bfs\in \mathcal{A}} |\qfsest - \qfs| \leq \sqrt{\frac{8}{n}\log \frac{2|\mathcal{A}|}{\delta}},$$
holds with probability at least $(1-\delta)$.
\end{lem}
Compared to the naive strategy, we get exponential improvements when $\mathcal{A}$ is compatible. In this case, with Lemma \ref{lem:compatible A fourier est}, the square loss of the Fourier estimations is less than $\beta^2=\frac{8|\mathcal{A}|}{n}\log \frac{2|\mathcal{A}|}{\delta}$ as needed in Theorem \ref{thm: QLD Predictor only}. Now, if $\mathcal{A}$ is not compatible, we need compatible covering that is explained in the next section.



\subsubsection{Compatible Covering}\label{subsec:compatible covering}
We proceed with extending the Fourier estimation process to general degree sets, consisting of incompatible measurements.  The idea is to cover the degree set $\mathcal{A}$ with compatible subsets as presented in Definition \ref{def: compatible degree set}. Moreover, we randomly partition the training samples into multiple batches one for each covering subset  $\mathcal{B}_j, j\in [m]$. We use samples from the $j$th batch to estimate $\qfs, \bfs\in \mathcal{B}_j$.  Let $n_j$ be the size of the $j$th batch. Among multiple coverings and choices of $n_j$'s, we chose those that minimize the square loss. In what follows, we first explain a way to find all coverings and derive bounds on the square loss. 


Finding compatible covers of $\mathcal{A}$ is a process solely depending on the structure of $\mathcal{A}$. Hence, it can be done once as a pre-processing step, independently of the samples. For that, we use an exhaustive search to find all possible compatible coverings of $\mathcal{A}$. The exhaustive search  involves checking the compatibility of the observables $M_{\bfs}, \bfs\in\mathcal{A}$.  From Proposition \ref{prop:compatible Ms},  we just need to check the commuting relation between  $\qps, \bfs\in \mathcal{A}$.  We  start with an observable $M_{\bfs}, \bfs\in \mathcal{A}$, hence creating a single-element subset $\set{M_{\bfs}}$. Next, we find a compatible ${M}_\bft, \bft \in \mathcal{A}\backslash \set{\bfs}$ and add it to	 $\set{M_{\bfs}}$.  We keep adding to the subset by finding observables that are compatible with all of its members. Once no more compatible observable is found, we create another subset by repeating this process for the remaining observables in $\mathcal{A}$.  
%In what follows, we explain a method to find a compatibility covering. 
 
%In addition to the compatible covering, we need to partition the training samples into multiple batches one for each covering subset  $\mathcal{B}_j, j\in [m]$.  Let $n_j$ be the size of the batch corresponding to $\mathcal{B}_j$ which will be determined later to minimize the square loss. %We will determine the batch sizes $n_j, j\in [m]$.

Next, we proceed with analyzing the square loss for each covering and sample partitioning. Since $\qfs, \bfs\in \mathcal{B}_j$ are estimated using the $j$th batch of samples, then from Lemma \ref{lem:compatible A fourier est}, we obtain a bound on the absolute difference {\small $\sup_{\bfs\in \mathcal{B}_j} |\qfsest - \qfs|.$}  With these bounds, the overall square loss is bounded as
\begin{align}\label{eq:qfs square loss}
\sum_{\bfs\in \mathcal{A}} (\qfsest-\qfs)^2 \leq \sum_{j=1}^m \frac{8|\mathcal{B}_j|}{n_j}\log \frac{2|\mathcal{B}_j|}{\delta}.
\end{align}
Hence, right-hand side in \eqref{eq:qfs square loss} gives an upper bound for $\beta^2$ as in Theorem \ref{thm: QLD Predictor only}. 
 Therefore, we choose the coverings $\mathcal{B}_j$ and batch sizes $n_j$ to minimize the above expression. For each covering,  the optimal batch sizes  $n_j$ are given in the following lemma.
 \begin{lem}\label{lem:optimal nj for covering }
 Having $n$ training samples and given  $\delta\in (0,1)$, the optimal batch sizes for a covering $\mathcal{B}_j, j\in[m]$  are given by $$n_j^* = n  \frac{\sqrt{|\mathcal{B}_j|\log( {2|\mathcal{B}_j|}/{\delta})}}{\sum_j \sqrt{|\mathcal{B}_j|\log( {2|\mathcal{B}_j|}/{\delta})}}.$$
 \end{lem} 
  \begin{proof}
 Let $x_j=\frac{n_j}{n}, j\in m$ and $b_j = |\mathcal{B}_j| \log(2{|\mathcal{B}_j|}/{\delta})$. The lemma follows by solving the optimization problem $$\min_{\bfx \in \RR^m} \sum_{j=1}^m \frac{b_j}{x_j},\quad  \text{subject to } x_j\geq 0, \text{ and } \sum_{j=1}^m x_j =1,$$  via Karush–Kuhn–Tucker (KKT) approach.
 \end{proof}
Therefore, by replacing $n_j^*$ into \eqref{eq:qfs square loss}, the right-hand side of \eqref{eq:qfs square loss} equals to $\Big(\sum_{j=1}^m \sqrt{ \frac{|\mathcal{B}_j|}{n}\log \frac{|\mathcal{B}_j|}{\delta}}\Big)^2$. As a result,  the best covering is the one that minimizes this quantity. With the optimal choice of covering and sample partitioning, we complete the estimation processes which is presented Procedure \ref{proc:FourierEstimation}. 
 Moreover, we establish Theorem \ref{thm: QLD general} by applying Theorem \ref{thm: QLD Predictor only} with 
$$\beta^2=\min_{\mathcal{B}_j \text{covering} of \mathcal{A}} \Big(\sum_{j=1}^m \sqrt{ \frac{|\mathcal{B}_j|}{n}\log \frac{|\mathcal{B}_j|}{\delta}}\Big)^2.$$


 \begin{procedure}[h]
\caption{FourierEstimation() in QLD algorithm}\label{proc:FourierEstimation}
\DontPrintSemicolon
 \SetKwProg{Fn}{Function}{:}{} 
 \SetKwProg{Est}{Estimation}{ (\emph{Batch} $j$, $\mathcal{B}_j$):}{}
 \Fn{\FourierEstimation{$\mathcal{B}_j, j\in [m]$}}{
 %Take the optimal covering of $\mathcal{A}$ denoted by $\mathcal{B}_j, j\in [m]$.\;
 Partition the samples into $m$ bathes, each of size $n_j^*, j\in [m]$, as in Lemma \ref{lem:optimal nj for covering }.\;
 
    \For{$j=1$ \KwTo $m$}{
 %%\Est{}{  
  \addvd{  On samples in the $j$th batch apply POVM $M^j_{ref}$ with operators  in \eqref{eq:Mref opt} and $\bfs_\ell\in \mathcal{B}_j$. \;}
%Apply $M^j_{ref}$ on each sample in the $j$th batch. \;
Compute the empirical Fourier coefficient $\qfsest$ for all $\bfs\in\mathcal{B}_j$,  as in \eqref{eq:qfsest compatible}. \;
   }
   \KwRet $\qfsest$ for all $\bfs\in\mathcal{A}$
   }
   
%\Fn{\FourierEstimation{$\mathcal{A}$}}{
% Construct the POVM $M_{ref}$ with operators as  in \eqref{eq:Mref opt}. \;
%Apply $M_{ref}$ on each sample. \;
%Compute the empirical Fourier coefficient $\qfsest$ for all $\bfs\in\mathcal{A}$,  as in \eqref{eq:qfsest compatible}. \;
%\KwRet $\qfsest, \bfs \in \mathcal{A}$\;
%}
\end{procedure} 

\addvd{Note that the running time of this procedure is $\order{n 4^{|\mathcal{A}|}}$, as there are $4^{|\mathcal{A}|}$ that many Fourier coefficients to estimate. Moreover, the running time of Algorithm \ref{alg: QLD general} is also dominated by this term.}   Lastly, we point out that in QLD algorithm, the set $\mathcal{A}$ is given as an input. Whether the optimal loss $\opt_{\mathcal{C}}$ of a concentrated class with degree set $\mathcal{A}$ is lower than another concentrated class with a different degree set is in general open. In the next section, we answer this question for a special type of concentrated measurement classes. 

==> app_useful_inequalities.tex <==
\section{Technical Norm and Trace Inequalities}\label{app:trace ineq}

Given $q>0$, the $q$-Schatten norm of an operator $A$ is defined as 
\begin{align*}
\norm{A}_{q} \deq \tr{\abs{A}^q}^{1/q}.
\end{align*}
% This norm is similar to the Schatten norm; however there is an  additional component which is the density operator $\rho$. One can see that for $q=2$, the above $\norm{A}_{2,\rho}$ reduces to the Schatten 2-norm of $A\sqrt{\rho}$. 
In what follows, we develop a number of useful properties for the $q$-norm above.  

\begin{proposition}\label{prop: trace ineq 1}
Given any density operator $\rho$, and a pair of bounded Hermitian operators $A$ and $B$, the following properties hold:
\begin{enumerate}[(a)]
\item $\norm{A+B}_{2}^2=\norm{A}^2_{2}+\norm{B}^2_{2}+2\tr{A^\dagger B}$
\item  $\tr{A B} \leq \norm{A}_{2}\norm{B}_{2}$
\item Minkowski inequality for $2$-norm : $\norm{A+B}_{2}\leq \norm{A}_{2}+\norm{B}_{2}$. 
%\item Minkowski inequality for $2$-norm : $\norm{A+B}_{2,\rho}\leq \norm{A}_{2,\rho}+\norm{B}_{2,\rho}$. 
\item  $\norm{A}_{1}\leq \norm{A}_{2}$. 
\end{enumerate}
\end{proposition} 
\begin{proof}
\noindent \textbf{(a):} Follows from the definition. 
%\begin{align*}
%\norm{A+B}_{2,\rho}^2 &= \tr{\big(A+B\big)^\dagger\big(A+B\big)\rho}\\
%& = \tr{\big(A^\dagger A + B^\dagger B +A^\dagger B + B^\dagger A \big)\rho}\\
%& = \norm{A}_{2,\rho}^2+\norm{B}_{2,\rho}^2 + 2\tr{A B \rho}. 
%\end{align*}
%Hence, the first statement is proved. 
\noindent \textbf{(b):} Follows from the noncommutative Cauchy-Schwarz inequality.  
%\begin{align*}
%\<A,B\>_\rho &= \tr{A^\dagger B \rho}=\tr{\big(\sqrt{\rho} A^\dagger\big) \big( B \sqrt{\rho}\big)}=\tr{\big( A\sqrt{\rho}\big)^\dagger \big( B \sqrt{\rho}\big)}\\
%&\leq \sqrt{\tr{\sqrt{\rho} A^\dagger A \sqrt{\rho}}\tr{\sqrt{\rho} B^\dagger B \sqrt{\rho}}}\\
%&=\sqrt{\tr{ A^\dagger A {\rho}}\tr{ B^\dagger B {\rho}}}=\norm{A}_{2,\rho}\norm{B}_{2,\rho}.
%\end{align*}

\noindent \textbf{(c):} Using (a) and (b) we can write:
\begin{align*}
\norm{A+B}_{2,\rho}^2 &= \norm{A}^2_{2,\rho}+\norm{B}^2_{2,\rho}+2\<A,B\>_\rho\\
& \leq  \norm{A}^2_{2,\rho}+\norm{B}^2_{2,\rho}+2\norm{A}_{2,\rho}\norm{B}_{2,\rho}\\
&=\Big(\norm{A}_{2,\rho}+\norm{B}_{2,\rho}\Big)^2
\end{align*}

\noindent \textbf{(d):} We have that $\norm{A}_{1,\rho} = \tr{|A|\rho}$. Since $A$ is Hermitian, it admits a \textit{spectral decomposition} as $A=\sum_i \mu_i\ketbra{\phi_i}$, where $\mu_i\in \RR$ and $\ket{\phi_i}$'s are an orthonormal basis.  Hence, $|A|$ admits the same decomposition but with $|\mu_i|$. Thus, we obtain that 
\begin{align*}
\norm{A}_{1,\rho} = \sum_j |\mu_j| \underbrace{\expectationvalue{\rho}{\phi_i}}_{\alpha_i},\qquad \norm{A}_{2,\rho} = \sqrt{\sum_j |\mu_j|^2 \expectationvalue{\rho}{\phi_i}}
 \end{align*}
As $\rho$ is a density operator, then $\alpha_i\in [0,1]$ and $\sum_i \alpha_i=1$. Hence, from the Jensen's inequality for square root function we have that 
\begin{align*}
\norm{A}_{2,\rho} = \sqrt{\sum_j |\mu_j|^2 \alpha_i} \geq \sum_j |\mu_j| \alpha_i = \norm{A}_{1,\rho}.
\end{align*}
%By definition 
%\begin{align*}
%\norm{A+B}_{1,\rho}&=  \tr{|A+B|\rho}\leq \sup_{U: unitary} |\tr{\big( |A+B|\big)\rho U}|
%\end{align*}
%From polar decomposition, there exists a unitary operator $V$ such that $(A+B)=V|A+B|$. Therefore,
%\begin{align*}
%\sup_{U}|\tr{\big( |A+B|\big)\rho U}| &= \sup_{U}|\tr{V^\dagger\big(A+B\big)\rho U}|\\
%&=\sup_{U}|\tr{\big(A+B\big)\rho U V^\dagger}|\\
%&\leq \sup_{W}|\tr{\big(A+B\big)\rho W}|\\
%& \leq \sup_{W}|\tr{A\rho W}|+ \sup_{W}|\tr{B\rho W}|
%\end{align*}
%\begin{align*}
%\tr{|A+B|\rho} &= \tr{U^\dagger (A+B)\rho}\leq \sup_{V: unitary}|\tr{(A+B)\rho V}|\\
%&\leq \sup_{V: unitary}|\tr{A\rho V}|+ \sup_{V: unitary}|\tr{B\rho V}|
%\end{align*}
 \end{proof}
 
 

From the Fourier expansion, we immediately get the following results. We omit the proof as they are straightforward. 
\begin{proposition}\label{prop:quantum Fourier properties}
Let $A, B \in \mathcal{B}(H_d)$ with Fourier coefficients $a_{\bfs}$ and $b_{\bfs}$, respectively. Then the following statements hold
\begin{enumerate}[(a)]
\item $\<A,B\>=\sum_{\bfs}a_{\bfs}^*b_{\bfs}$. Hence, Parseval's identity holds: $\norm{A}_2^2=\sum_{\bfs} |a_{\bfs}|^2$. 
\item If $A$ is Hermitian, then $a_{\bfs}$ are real. 
%\item If $A$ is a quantum Boolean operator, then $\norm{A}_\infty=\norm{A}_q=1$.
\end{enumerate}
\end{proposition}
%\begin{proof}
%The first statement is straightforward as $\qps$ are orthogonal. (b) follows  from the uniqueness of $a_{\bfs}$ and that $\qps$ are Hermitian. Lastly, (c) is due to (a) and the fact that $\<A,A\> = 1$ when $A$ is Boolean. 
%\end{proof}
%\begin{fact}\label{fact:boolean opt norm}
%If $A \in \mathcal{B}(H_d)$ is a quantum Boolean operator, then $\norm{A}_\infty=\norm{A}_q=1$. 
%\end{fact} 


==> proof_lem_estimating_qfs.tex <==
%\section{Proof of Lemma \ref{lem:estimating one qfs}}\label{app:lem:estimating one qfs}
\begin{proof}
Note that the conditional expectation of $Z_i$ given the $i$th sample $\hat{\rho}_{y_i}\tensor \ketbra{y_i}$ can be written as 
\begin{align*}
\EE[Z_i| \hat{\rho}_{y_i}\tensor \ketbra{y_i}] = \sum_{z\in\pmm} z~ \tr{\Msopt_z \big(\hat{\rho}_{y_i}\tensor \ketbra{y_i}\big)}.
\end{align*}
Note that the above value in fact is the \textit{expectation value} of the observable $M_{\bfs}$ in state $\hat{\rho}_{y_i}\tensor \ketbra{y_i}$. With that the overall expectation of $Z_i$ equals 
\begin{align*}
 \EE[Z_i]&=\sum_{y\in \mathcal{Y}}\sum_{z\in\pmm} z~ p_{y} \tr{\Msopt_z \big(\hat{\rho}_{y}\tensor \ketbra{y}\big)}\\
  &=\sum_{z\in\pmm} z ~\tr{\Msopt_z \rho_{XY}}\\
  & =  \Tr{\big( \Msopt_1 - \Msopt_{-1}\big) \rho_{XY}}\\
  & =  \Tr{\qps \qfY\rho_{XY}}
 \end{align*} 
 where we used the linearity of the trace and \eqref{eq:Ms operators}. Hence, the proof is complete as the right-hand side is $\qfs$.
\end{proof}

==> proof_prop_quantum_fourier.tex <==
%\section{ Proof of Proposition \ref{prop:quantum Fourier}}\label{app:proof:prop:quantum Fourier}
\begin{proof}
We start with $d=1$. Note that $\set{\outerproduct{\ell}{k}: \ell,k\in \set{0,1}}$ is the standard basis for all operators on $H_1$. Hence, it suffices to write $\outerproduct{\ell}{k}$ in terms of the Pauli operators. For any $k\neq \ell\in \set{0,1}$ we have that
\begin{align*}
\outerproduct{\ell}{\ell}=\frac{1}{2}\sigma^0 + \frac{1}{2}(-1)^\ell\sigma^3, \qquad \outerproduct{\ell}{k} = \frac{1}{2}\sigma^1 + \frac{1}{2}(-1)^\ell i\sigma^3,
\end{align*}
where $i\in \CC$ with $i^2=-1$. This completes the proof for $d=1$. For $d>1$, the set of all $d$-fold tensor product of $\outerproduct{\ell}{k}$'s is the standard basis for $\mathcal{B}(H_d)$. Hence, from the above relations, such basis elements can be written as a linear combinations of $\qps, \bfs\in \set{0,1}^d$. That completes the proof for $d>1$. The uniqueness follows as $\qps$ are orthogonal.  
\end{proof}

==> proof_thm_Junta.tex <==
% \subsection{Proof of Theorem \ref{thm: Kjunta sample complexity}}\label{proof:thm: Kjunta sample complexity}

% The main ingredient in the proof of this theorem is the following lemma which is proved in Appendix \ref{proof:lem:norm2 sign}.
 

 \begin{lem}\label{lem:norm2 sign}
Let $\mathcal{M}_{\mathcal{J}}$ be a measurement depending on only the coordinates $\mathcal{J}\subset [d]$ where its operator representation is $\gm=\sign[\BJ]$ for some Hermitian operator $\BJ$ depending only on the coordinates of $\mathcal{J}$. Then,
\begin{align*}
\Loss(\mathcal{M}_{\mathcal{J}})&\leq \frac{1}{2}\Big(1-\norm{\qYJ}_{1,\rho}\Big)+U\Big(\norm{\qYJ-\BJ}_{2,\rho}\Big),
\end{align*}
where $U(x)=x^3+\frac{3}{2}x^2+\frac{5}{4}x$, for all $x\geq 0$.
\end{lem}
%Having this lemma, the proof of the theorem is as follows. We run FourierEstimation{$\mathcal{B}_j, j\in [m]$}, where $\mathcal{B}_j$'s are the optimal covering of the degree set $\mathcal{A}=\big\{\bfs\in \set{0,1,2,3}^d: |\supp(\bfs)|\leq k\big\}$. As a result, we obtain estimated Fourier coefficients $\qfs, \bfs\in \mathcal{A}$, with square loss satisfying the following inequality with probability $(1-\delta)$
%\begin{align}\label{eq:juynta qfest}
%\sum_{\bfs: |\supp(\bfs)|\leq k} (\qfs-\qfsest)^2\leq \epsilon'_n := \min_{\mathcal{B}_j~\text{covering of}~ \mathcal{A}}\Big( \sum_{j=1}^m \sqrt{ \frac{|\mathcal{B}_j|}{n}\log \frac{|\mathcal{B}_j|}{\delta}}\Big)^2.
%\end{align}
Given this result, suppose $\qfsest$ are  the estimated Pauli coefficients.  Then,  
For any $\mathcal{J}$, define the operator $\qfYestJ = \sum_{\bfs: \supp(\bfs)\subseteq \mathcal{J}} \qfsest \qps$ and let $\mathcal{M}$ be the measurement whose operator representation is $\gm=\sign[\qfYestJ]$. Then, from Lemma \ref{lem:norm2 sign} we have that 
\begin{align*}
\Loss(\mathcal{M}) &\leq \frac{1}{2}\Big(1-\norm{\qYJ}_{1,\rho}\Big)+U\Big(\norm{\qYJ-\qfYestJ}_{2,\rho}\Big).
\end{align*}
Next, we bound the second term in the right-hand side. From Parseval's identity (Proposition \ref{prop:quantum Fourier properties} in Appendix \ref{app:trace ineq}) and \eqref{eq:juynta qfest} we obtain that 
\begin{align*}
\norm{\qYJ-\qfYestJ}_{2,\rho}^2=\sum_{\bfs: \supp(\bfs)\subseteq \mathcal{J}} (\qfs-\qfsest)^2\leq \epsilon'_n ,
\end{align*}
which implies that $\Loss(\mathcal{M}) \leq \frac{1}{2}\big(1-\norm\big{\qYJ}_{1,\rho}\big)+U(\sqrt{\epsilon'_n }).$ Next, we search over all $\mathcal{J}$ with $k$ elements and find the one that maximizes $\norm\big{\qfYestJ}_{1,\rho}$. Let $\hat{\mathcal{J}}$ be such a subset and $\hat{\mathcal{M}}$ be the measurement with $G_{\hat{{M}}} =\sign[{\qfYest}^{\subseteq \hat{\mathcal{J}}}]$.  Then 
\begin{align}\label{eq:Loss M up 1}
\Loss(\hat{\mathcal{M}})&\leq \frac{1}{2}\big(1-\norm\big{{\qfY}^{\subseteq \hat{\mathcal{J}}}}_{1,\rho}\big)+U(\sqrt{\epsilon'_n}).
\end{align}
In what follows, we show that the right-hand side is less than $\opt(k) +\sqrt{\epsilon'_n }+ U(\sqrt{\epsilon'_n })$.
Note that form the triangle inequality and Jensen's inequality (Proposition \ref{prop: trace ineq 1}) for any $\mathcal{J}$, we have that
\begin{align*}
\Big|~\norm\big{\qfYestJ}_{1,\rho}- \norm\big{\qYJ}_{1,\rho}\Big| &\leq \norm\big{\qYJ-\qfYestJ}_{1,\rho}\\
& \leq \norm\big{\qYJ-\qfYestJ}_{2,\rho}\\
& \leq  \sqrt{\epsilon'_n}.
\end{align*}
Let $\mathcal{J}^*=\argmax_{\mathcal{J}: |\mathcal{J}|=k} \norm\big{\qYJ}_{1,\rho}$. Then
\begin{align*}
\norm\big{{\qfY}^{\subseteq \hat{\mathcal{J}}}}_{1,\rho} &\geq \norm\big{{\qfYest}^{\subseteq \hat{\mathcal{J}}}}_{1,\rho} -\sqrt{\epsilon'_n} \geq \norm\big{{\qfYest}^{\subseteq \mathcal{J}^*}}_{1,\rho} -\sqrt{\epsilon'_n} \geq \norm\big{{\qfY}^{\subseteq \mathcal{J}^*}}_{1,\rho} -2\sqrt{\epsilon'_n}.
\end{align*}
As a result, using \eqref{eq:Loss M up 1}, we have that
\begin{align*}
\Loss(\hat{\mathcal{M}})&\leq \frac{1}{2}\big(1-\norm{{\qfY}^{\subseteq \mathcal{J}^*}}_{1,\rho} +2\sqrt{\epsilon'_n}\big)+U(\sqrt{\epsilon'_n})\\
&=\opt(k) +\sqrt{\epsilon'_n} + U(\sqrt{\epsilon'_n}),
\end{align*}
where the last equality follows from Lemma \ref{lem: k junta opt}. The proof is complete by noting that $ U(x)\leq 4x$, for any $x\in [0,1]$. This implies that $\Loss(\hat{\mathcal{M}})\leq \opt(k)+5\sqrt{\epsilon'_n}$. 
%The proof is complete by replacing the $\epsilon'_n$ with the right-hand side of \eqref{eq:pstar-Piest}. 


